On The Effect Of Code Review On Code Smells

Code smells are symptoms of poor design quality. Since code review is a process that also aims at improving code quality, we investigate whether and how code review influences the severity of code smells. In this study, we analyze more than 21,000 code reviews belonging to seven Java open-source projects; we find that active and participated code reviews have a significant influence on the likelihood of reducing the severity of code smells. This result seems to confirm the expectations around code review's influence on code quality. However, by manually investigating 365 cases in which the severity of a code smell in a file was reduced with a review, we found that-in 95% of the cases-the reduction was a side effect of changes that reviewers requested on matters unrelated to code smells. Data and materials [https://doi.org/10.5281/zenodo.3588501].

==> sections/threats.tex <==
% !TEX root = ../main.tex
% !TeX spellcheck = en_US	
	\section{Threats to Validity}
	\label{sec:threats}
	
	TBD
